Transferring Visual Attributes from Natural Language to Verified Image Generation

Text to image generation methods (T2I) are widely popular in generating art and other creative artifacts. While visual hallucinations can be a positive factor in scenarios where creativity is appreciated, such artifacts are poorly suited for cases where the generated image needs to be grounded in complex natural language without explicit visual elements. In this paper, we propose to strengthen the consistency property of T2I methods in the presence of natural complex language, which often breaks the limits of T2I methods by including non-visual information, and textual elements that require knowledge for accurate generation. To address these phenomena, we propose a Natural Language to Verified Image generation approach (NL2VI) that converts a natural prompt into a visual prompt, which is more suitable for image generation. A T2I model then generates an image for the visual prompt, which is then verified with VQA algorithms. Experimentally, aligning natural prompts with image generation can improve the consistency of the generated images by up to 11% over the state of the art. Moreover, improvements can generalize to challenging domains like cooking and DIY tasks, where the correctness of the generated image is crucial to illustrate actions.

==> Aligning_Natural_Prompts_and_Image_Generation/tables/question_distribution.tex <==
% % Please add the following required packages to your document preamble:
% % \usepackage{multirow}
% \begin{table*}[h]
% \centering
% \begin{tabular}{lccc}
% \toprule
%  &
%   \textbf{\# Questions} &
%   \textbf{\begin{tabular}[c]{@{}c@{}}\# Questions\\ (Filtered)\end{tabular}} &
%   \textbf{\begin{tabular}[c]{@{}c@{}}\% Questions\\ (Filtered)\end{tabular}} \\ \midrule
% \textbf{Recipes}\\
% \midrule
% \quad Binary Questions    & 392 & 386 & 98.4 \\
% \quad Open-Ended Questions & 233 & 174 & 74.7\\
% \quad Total & 625 & 560 & 89.6\\ \midrule
% \textbf{Wikihow}\\
% \midrule
% \quad Binary Questions     & 403 & 388 & 96.3 \\
% \quad Open-Ended Questions& 222 & 158 & 71.1 \\ 
% \quad Total & 625 & 546 & 87.4\\ 
% \bottomrule
% \end{tabular}
% \caption{Distribution of generated questions for the Recipes and WikiHow datasets before and after filtering (UnifiedQA).}
% \label{tab:question-distribution}
% \end{table*}

\begin{table}[h]
\centering
\begin{tabular}{lcc}
\toprule
 &
  \textbf{\begin{tabular}[c]{@{}c@{}}Generated\\ Questions\end{tabular}} &
  \textbf{\begin{tabular}[c]{@{}c@{}}Verified\\ Questions\end{tabular}} \\ \midrule
\textbf{Recipes}\\
\midrule
\quad Binary    & 392 & 386 \\
\quad Open-Ended & 233 & 174 \\
\midrule
\textbf{Wikihow}\\
\midrule
\quad Binary      & 403 & 388 \\
\quad Open-Ended  & 222 & 158 \\ 
\bottomrule
\end{tabular}
\caption{Distribution of generated questions for the Recipes and WikiHow datasets before and after filtering (UnifiedQA).}
\label{tab:question-distribution}
\end{table}



==> Aligning_Natural_Prompts_and_Image_Generation/tables/question_filtering.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
% \usepackage{multirow}
\begin{table*}[h]
\centering
\begin{tabular}{@{}l|cc|cc|cc@{}}
\toprule
 & \multicolumn{2}{c|}{\textbf{\% of valid questions}} & \multicolumn{2}{c|}{\textbf{Precision}} & \multicolumn{2}{c}{\textbf{Recall}} \\ \midrule
\textbf{Question filtering}  & \textbf{Recipes}         & \textbf{Wikihow}        & \textbf{Recipes}       & \textbf{Wikihow}     & \textbf{Recipes}     & \textbf{Wikihow}   \\ \midrule
QANLU                       & 50.4                     & 50.8                    & 22.2                   & 33.3                  & 28.6                 & 28.6               \\
Unified-QA                  & 89.6                     & 87.8                    & 90.9                   & 84.2                  & 71.4                 & 76.2               \\ \bottomrule
\end{tabular}
\caption{\label{tab:question-filtering-table}Evaluation of the question filtering stage.}
\end{table*}


% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
% \usepackage{multirow}


==> Aligning_Natural_Prompts_and_Image_Generation/tables/vfc_accuracy.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
% \usepackage{multirow}
\begin{table}[t]
    \small
    \begin{tabular}{@{}lll|c|c@{}}
        \toprule
        \textbf{Models} & \textbf{LLM} & \textbf{VQA} & \textbf{Recipes} & \textbf{Wikihow} \\\midrule
        CLIPScore  & n/a     & n/a     & 57.4                        & 53.8                       \\
        TIFA     & GPT-3.5  & mPLUG   & 72.5                        & 64.9                 \\
        NL2VI      & PaLM    & OFA    & 78.4                        & 73.6                  \\
        NL2VI      & GPT-3.5  & PaLI    & 80.3                        & 76.0                  \\
        \bottomrule
    \end{tabular}
    \centering
    \caption{\label{tab:vfc-accuracy-table} Human evaluation of the different visual factual consistency methods.}
\end{table}




==> Aligning_Natural_Prompts_and_Image_Generation/tables/visual_prompts.tex <==
\begin{table}[t]
        \centering
        \begin{tabular}{@{}l|cccc@{}}
            \toprule
            \multirow{2}{*}{\textbf{Models}}  & \multicolumn{2}{c}{\textbf{Recipes}} & \multicolumn{2}{c}{\textbf{Wikihow}} \\
                           & AUC   &   P@1      & AUC     &  P@1   \\  \midrule
            PaLM           & 82.5  &   42.0     & 90.2    &  56.0  \\
            GPT-3.5        & 92.8  &   74.0     & 94.9    &  80.0  \\
            \bottomrule
        \end{tabular}
        \captionof{table}{Alignment between natural language prompts and visual generation prompts. }
        \label{visual-prompts-table}
\end{table}

